Flattened Catalan Words

In this work, we define flattened Catalan words as Catalan words whose runs of weak ascents have leading terms that appear in weakly increasing order. We provide generating functions, formulas, and asymptotic expressions for the number of flattened Catalan words based on the number of runs of ascents (descents), runs of weak ascents (descents), $\ell$-valleys, valleys, symmetric valleys, $\ell$-peaks, peaks, and symmetric peaks.

==> Figures/flatcatlength4with3runsofdescents.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da45619059610413315] 
\draw    (141.95,59.86) -- (168.89,59.82) ;
%Straight Lines [id:da15461034972270649] 
\draw    (220.59,35.07) -- (246,35.07) ;
%Straight Lines [id:da061772920472648374] 
\draw    (194.95,59.82) -- (220.37,59.82) ;
%Straight Lines [id:da9584101167426982] 
\draw    (169.11,35.07) -- (194.52,35.07) ;
%Straight Lines [id:da18720613126653418] 
\draw    (168.89,59.82) -- (169.11,35.07) ;
%Straight Lines [id:da0361201254574921] 
\draw    (194.95,59.82) -- (195.17,35.07) ;
%Straight Lines [id:da9340106130665808] 
\draw    (220.37,59.82) -- (220.59,35.07) ;
%Shape: Ellipse [id:dp9834798522276142] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (140,59.86) .. controls (140,58.86) and (140.88,58.05) .. (141.95,58.05) .. controls (143.03,58.05) and (143.91,58.86) .. (143.91,59.86) .. controls (143.91,60.86) and (143.03,61.67) .. (141.95,61.67) .. controls (140.88,61.67) and (140,60.86) .. (140,59.86) -- cycle ;
%Shape: Ellipse [id:dp42987655676415193] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (166.28,59.82) .. controls (166.28,58.82) and (167.16,58.01) .. (168.24,58.01) .. controls (169.32,58.01) and (170.19,58.82) .. (170.19,59.82) .. controls (170.19,60.82) and (169.32,61.63) .. (168.24,61.63) .. controls (167.16,61.63) and (166.28,60.82) .. (166.28,59.82) -- cycle ;
%Shape: Ellipse [id:dp9076659699280633] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (167.16,35.21) .. controls (167.08,34.21) and (167.89,33.35) .. (168.96,33.27) .. controls (170.04,33.2) and (170.98,33.94) .. (171.06,34.94) .. controls (171.14,35.94) and (170.33,36.8) .. (169.25,36.88) .. controls (168.17,36.95) and (167.24,36.2) .. (167.16,35.21) -- cycle ;
%Shape: Ellipse [id:dp5822815528776909] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (193.22,35.07) .. controls (193.22,34.08) and (194.09,33.27) .. (195.17,33.27) .. controls (196.25,33.27) and (197.13,34.08) .. (197.13,35.07) .. controls (197.13,36.07) and (196.25,36.88) .. (195.17,36.88) .. controls (194.09,36.88) and (193.22,36.07) .. (193.22,35.07) -- cycle ;
%Shape: Ellipse [id:dp602977084437603] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (193,59.82) .. controls (193,58.82) and (193.88,58.01) .. (194.95,58.01) .. controls (196.03,58.01) and (196.91,58.82) .. (196.91,59.82) .. controls (196.91,60.82) and (196.03,61.63) .. (194.95,61.63) .. controls (193.88,61.63) and (193,60.82) .. (193,59.82) -- cycle ;
%Shape: Ellipse [id:dp9818663230677074] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (218.41,59.82) .. controls (218.41,58.82) and (219.29,58.01) .. (220.37,58.01) .. controls (221.45,58.01) and (222.32,58.82) .. (222.32,59.82) .. controls (222.32,60.82) and (221.45,61.63) .. (220.37,61.63) .. controls (219.29,61.63) and (218.41,60.82) .. (218.41,59.82) -- cycle ;
%Shape: Ellipse [id:dp800390397059647] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (218.63,35.07) .. controls (218.63,34.08) and (219.51,33.27) .. (220.59,33.27) .. controls (221.67,33.27) and (222.54,34.08) .. (222.54,35.07) .. controls (222.54,36.07) and (221.67,36.88) .. (220.59,36.88) .. controls (219.51,36.88) and (218.63,36.07) .. (218.63,35.07) -- cycle ;
%Shape: Ellipse [id:dp8376520854919951] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (242.09,35.07) .. controls (242.09,34.08) and (242.97,33.27) .. (244.05,33.27) .. controls (245.12,33.27) and (246,34.08) .. (246,35.07) .. controls (246,36.07) and (245.12,36.88) .. (244.05,36.88) .. controls (242.97,36.88) and (242.09,36.07) .. (242.09,35.07) -- cycle ;
%Straight Lines [id:da35575303041173467] 
\draw    (11.95,59.86) -- (38.89,59.82) ;
%Straight Lines [id:da33100658957201845] 
\draw    (64.59,35.07) -- (90,35.07) ;
%Straight Lines [id:da24971304898918156] 
\draw    (88.95,59.82) -- (114.37,59.82) ;
%Straight Lines [id:da3906063265609738] 
\draw    (38.24,60.01) -- (63.65,60.01) ;
%Straight Lines [id:da8529797797737865] 
\draw    (64.37,59.82) -- (64.59,35.07) ;
%Shape: Ellipse [id:dp5353888133664858] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (10,59.86) .. controls (10,58.86) and (10.88,58.05) .. (11.95,58.05) .. controls (13.03,58.05) and (13.91,58.86) .. (13.91,59.86) .. controls (13.91,60.86) and (13.03,61.67) .. (11.95,61.67) .. controls (10.88,61.67) and (10,60.86) .. (10,59.86) -- cycle ;
%Shape: Ellipse [id:dp24435995713929592] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (36.28,59.82) .. controls (36.28,58.82) and (37.16,58.01) .. (38.24,58.01) .. controls (39.32,58.01) and (40.19,58.82) .. (40.19,59.82) .. controls (40.19,60.82) and (39.32,61.63) .. (38.24,61.63) .. controls (37.16,61.63) and (36.28,60.82) .. (36.28,59.82) -- cycle ;
%Shape: Ellipse [id:dp9036608717386274] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (63,59.82) .. controls (63,58.82) and (63.88,58.01) .. (64.95,58.01) .. controls (66.03,58.01) and (66.91,58.82) .. (66.91,59.82) .. controls (66.91,60.82) and (66.03,61.63) .. (64.95,61.63) .. controls (63.88,61.63) and (63,60.82) .. (63,59.82) -- cycle ;
%Shape: Ellipse [id:dp8655420717426889] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (86.41,59.82) .. controls (86.41,58.82) and (87.29,58.01) .. (88.37,58.01) .. controls (89.45,58.01) and (90.32,58.82) .. (90.32,59.82) .. controls (90.32,60.82) and (89.45,61.63) .. (88.37,61.63) .. controls (87.29,61.63) and (86.41,60.82) .. (86.41,59.82) -- cycle ;
%Shape: Ellipse [id:dp04522047002769991] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (62.63,35.07) .. controls (62.63,34.08) and (63.51,33.27) .. (64.59,33.27) .. controls (65.67,33.27) and (66.54,34.08) .. (66.54,35.07) .. controls (66.54,36.07) and (65.67,36.88) .. (64.59,36.88) .. controls (63.51,36.88) and (62.63,36.07) .. (62.63,35.07) -- cycle ;
%Shape: Ellipse [id:dp2032444226236726] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (86.09,35.07) .. controls (86.09,34.08) and (86.97,33.27) .. (88.05,33.27) .. controls (89.12,33.27) and (90,34.08) .. (90,35.07) .. controls (90,36.07) and (89.12,36.88) .. (88.05,36.88) .. controls (86.97,36.88) and (86.09,36.07) .. (86.09,35.07) -- cycle ;
%Straight Lines [id:da627747553768172] 
\draw    (88.37,59.82) -- (88.59,35.07) ;
%Shape: Ellipse [id:dp9661169002704324] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (113.41,59.82) .. controls (113.41,58.82) and (114.29,58.01) .. (115.37,58.01) .. controls (116.45,58.01) and (117.32,58.82) .. (117.32,59.82) .. controls (117.32,60.82) and (116.45,61.63) .. (115.37,61.63) .. controls (114.29,61.63) and (113.41,60.82) .. (113.41,59.82) -- cycle ;
%Straight Lines [id:da7458400654853977] 
\draw    (272.95,60.86) -- (299.89,60.82) ;
%Straight Lines [id:da1774190792280398] 
\draw    (351.59,36.07) -- (377,36.07) ;
%Straight Lines [id:da3692178116699204] 
\draw    (326.95,9.82) -- (352.37,9.82) ;
%Straight Lines [id:da30157137978582316] 
\draw    (300.11,36.07) -- (325.52,36.07) ;
%Straight Lines [id:da22565393124139443] 
\draw    (299.89,60.82) -- (300.11,36.07) ;
%Straight Lines [id:da7174077844825498] 
\draw    (326.17,34.27) -- (326.39,9.52) ;
%Straight Lines [id:da010212848625338] 
\draw    (351.37,35.82) -- (351.59,11.07) ;
%Shape: Ellipse [id:dp8808927460566724] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (271,60.86) .. controls (271,59.86) and (271.88,59.05) .. (272.95,59.05) .. controls (274.03,59.05) and (274.91,59.86) .. (274.91,60.86) .. controls (274.91,61.86) and (274.03,62.67) .. (272.95,62.67) .. controls (271.88,62.67) and (271,61.86) .. (271,60.86) -- cycle ;
%Shape: Ellipse [id:dp1701065005362381] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (297.28,60.82) .. controls (297.28,59.82) and (298.16,59.01) .. (299.24,59.01) .. controls (300.32,59.01) and (301.19,59.82) .. (301.19,60.82) .. controls (301.19,61.82) and (300.32,62.63) .. (299.24,62.63) .. controls (298.16,62.63) and (297.28,61.82) .. (297.28,60.82) -- cycle ;
%Shape: Ellipse [id:dp6264491978037556] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (298.16,36.21) .. controls (298.08,35.21) and (298.89,34.35) .. (299.96,34.27) .. controls (301.04,34.2) and (301.98,34.94) .. (302.06,35.94) .. controls (302.14,36.94) and (301.33,37.8) .. (300.25,37.88) .. controls (299.17,37.95) and (298.24,37.2) .. (298.16,36.21) -- cycle ;
%Shape: Ellipse [id:dp21585792104364543] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (324.22,36.07) .. controls (324.22,35.08) and (325.09,34.27) .. (326.17,34.27) .. controls (327.25,34.27) and (328.13,35.08) .. (328.13,36.07) .. controls (328.13,37.07) and (327.25,37.88) .. (326.17,37.88) .. controls (325.09,37.88) and (324.22,37.07) .. (324.22,36.07) -- cycle ;
%Shape: Ellipse [id:dp31900140257282106] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (325,9.82) .. controls (325,8.82) and (325.88,8.01) .. (326.95,8.01) .. controls (328.03,8.01) and (328.91,8.82) .. (328.91,9.82) .. controls (328.91,10.82) and (328.03,11.63) .. (326.95,11.63) .. controls (325.88,11.63) and (325,10.82) .. (325,9.82) -- cycle ;
%Shape: Ellipse [id:dp5008460190855946] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (349.41,35.82) .. controls (349.41,34.82) and (350.29,34.01) .. (351.37,34.01) .. controls (352.45,34.01) and (353.32,34.82) .. (353.32,35.82) .. controls (353.32,36.82) and (352.45,37.63) .. (351.37,37.63) .. controls (350.29,37.63) and (349.41,36.82) .. (349.41,35.82) -- cycle ;
%Shape: Ellipse [id:dp04874662759431325] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (349.63,10.07) .. controls (349.63,9.08) and (350.51,8.27) .. (351.59,8.27) .. controls (352.67,8.27) and (353.54,9.08) .. (353.54,10.07) .. controls (353.54,11.07) and (352.67,11.88) .. (351.59,11.88) .. controls (350.51,11.88) and (349.63,11.07) .. (349.63,10.07) -- cycle ;
%Shape: Ellipse [id:dp6269268577714247] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (373.09,36.07) .. controls (373.09,35.08) and (373.97,34.27) .. (375.05,34.27) .. controls (376.12,34.27) and (377,35.08) .. (377,36.07) .. controls (377,37.07) and (376.12,37.88) .. (375.05,37.88) .. controls (373.97,37.88) and (373.09,37.07) .. (373.09,36.07) -- cycle ;
%Straight Lines [id:da505533528207223] 
\draw    (403.95,61.86) -- (430.89,61.82) ;
%Straight Lines [id:da5780779858128964] 
\draw    (457.95,10.82) -- (483.37,10.82) ;
%Straight Lines [id:da455451030775063] 
\draw    (431.11,37.07) -- (456.52,37.07) ;
%Straight Lines [id:da3129979048046335] 
\draw    (430.89,61.82) -- (431.11,37.07) ;
%Straight Lines [id:da1485547502943535] 
\draw    (457.17,35.27) -- (457.39,10.52) ;
%Straight Lines [id:da16470088703058094] 
\draw    (482.37,36.82) -- (482.59,12.07) ;
%Shape: Ellipse [id:dp32573679531753674] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (402,61.86) .. controls (402,60.86) and (402.88,60.05) .. (403.95,60.05) .. controls (405.03,60.05) and (405.91,60.86) .. (405.91,61.86) .. controls (405.91,62.86) and (405.03,63.67) .. (403.95,63.67) .. controls (402.88,63.67) and (402,62.86) .. (402,61.86) -- cycle ;
%Shape: Ellipse [id:dp8545732487648943] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (428.28,61.82) .. controls (428.28,60.82) and (429.16,60.01) .. (430.24,60.01) .. controls (431.32,60.01) and (432.19,60.82) .. (432.19,61.82) .. controls (432.19,62.82) and (431.32,63.63) .. (430.24,63.63) .. controls (429.16,63.63) and (428.28,62.82) .. (428.28,61.82) -- cycle ;
%Shape: Ellipse [id:dp2819301698951193] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (429.16,37.21) .. controls (429.08,36.21) and (429.89,35.35) .. (430.96,35.27) .. controls (432.04,35.2) and (432.98,35.94) .. (433.06,36.94) .. controls (433.14,37.94) and (432.33,38.8) .. (431.25,38.88) .. controls (430.17,38.95) and (429.24,38.2) .. (429.16,37.21) -- cycle ;
%Shape: Ellipse [id:dp03236301245298756] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (455.22,37.07) .. controls (455.22,36.08) and (456.09,35.27) .. (457.17,35.27) .. controls (458.25,35.27) and (459.13,36.08) .. (459.13,37.07) .. controls (459.13,38.07) and (458.25,38.88) .. (457.17,38.88) .. controls (456.09,38.88) and (455.22,38.07) .. (455.22,37.07) -- cycle ;
%Shape: Ellipse [id:dp06803854033372647] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (456,10.82) .. controls (456,9.82) and (456.88,9.01) .. (457.95,9.01) .. controls (459.03,9.01) and (459.91,9.82) .. (459.91,10.82) .. controls (459.91,11.82) and (459.03,12.63) .. (457.95,12.63) .. controls (456.88,12.63) and (456,11.82) .. (456,10.82) -- cycle ;
%Shape: Ellipse [id:dp6595699553110621] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (480.41,36.82) .. controls (480.41,35.82) and (481.29,35.01) .. (482.37,35.01) .. controls (483.45,35.01) and (484.32,35.82) .. (484.32,36.82) .. controls (484.32,37.82) and (483.45,38.63) .. (482.37,38.63) .. controls (481.29,38.63) and (480.41,37.82) .. (480.41,36.82) -- cycle ;
%Shape: Ellipse [id:dp022334562086833154] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (480.63,11.07) .. controls (480.63,10.08) and (481.51,9.27) .. (482.59,9.27) .. controls (483.67,9.27) and (484.54,10.08) .. (484.54,11.07) .. controls (484.54,12.07) and (483.67,12.88) .. (482.59,12.88) .. controls (481.51,12.88) and (480.63,12.07) .. (480.63,11.07) -- cycle ;
%Straight Lines [id:da52677851613598] 
\draw    (482.59,62.07) -- (508,62.07) ;
%Straight Lines [id:da8188465998370857] 
\draw    (482.37,61.82) -- (482.59,37.07) ;
%Shape: Ellipse [id:dp697293986459808] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (480.41,61.82) .. controls (480.41,60.82) and (481.29,60.01) .. (482.37,60.01) .. controls (483.45,60.01) and (484.32,60.82) .. (484.32,61.82) .. controls (484.32,62.82) and (483.45,63.63) .. (482.37,63.63) .. controls (481.29,63.63) and (480.41,62.82) .. (480.41,61.82) -- cycle ;
%Shape: Ellipse [id:dp6131945064334119] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (507.41,61.82) .. controls (507.41,60.82) and (508.29,60.01) .. (509.37,60.01) .. controls (510.45,60.01) and (511.32,60.82) .. (511.32,61.82) .. controls (511.32,62.82) and (510.45,63.63) .. (509.37,63.63) .. controls (508.29,63.63) and (507.41,62.82) .. (507.41,61.82) -- cycle ;

% Text Node
\draw (122,145.4) node [anchor=north west][inner sep=0.75pt]    {};


\end{tikzpicture}
